Learning Stable and Passive Neural Differential Equations

In this paper, we introduce a novel class of neural differential equation, which are intrinsically Lyapunov stable, exponentially stable or passive. We take a recently proposed Polyak Lojasiewicz network (PLNet) as an Lyapunov function and then parameterize the vector field as the descent directions of the Lyapunov function. The resulting models have a same structure as the general Hamiltonian dynamics, where the Hamiltonian is lower- and upper-bounded by quadratic functions. Moreover, it is also positive definite w.r.t. either a known or learnable equilibrium. We illustrate the effectiveness of the proposed model on a damped double pendulum system.

==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Removed from the main
% \begin{itemize}
% \item Hamiltonian system
% 
% \end{itemize}
% \subsubsection{Hamiltonian dyanmics and port Hamiltonian system:}
% The standard Hamiltonian dynamics can be written as: 
% \begin{equation}
% \begin{aligned}
% \dot{q} &= \frac{\partial H}{\partial p} (q, p), \\
% \dot{p} &= -\frac{\partial H}{\partial q} (q, p) + F
% \end{aligned}
% \end{equation}
% where $H(q, p)$ is the Hamiltonian, representing the total energy of the system, $F$ is the generalized force input, $q$ and $p$ are generalized coordinates and momenta\cite{van2014port}. 

% Considering the input and output, one can extend Hamiltonian dynamics to the standard input-state-output port-Hamiltonian system model: 
% \begin{equation}\label{eq:pH}
%     \begin{split}
%         \dot x &= (J(x)- R(x))\nabla H(x) + g(x)u \\
%         y &= g(x)^\top \nabla H(x)
%     \end{split}
% \end{equation}
% where $u$, $y$ are the input–output pairs, $J(x) = - J(x) ^\top$ is the structure matrix, $R = R^\top \geq 0$ is the resistive matrix, and $H(x)$ is the scalar Hamiltonian function. In general, $H(x)$ describes the internal energy distribution within the system. $J(x)$ reflects the energy flux and $R(x)$ specifies the internal energy dissipation.  
 % \subsubsection{Learning stable neural dynamics}

% The learnt dynamical model is defined via \eqref{eq:f_proj}:
% \begin{equation}
% \label{eq:f_proj}
% \begin{aligned}
% f(x)
% = \hat{f}(x) - \nabla V(x)\frac{\text{ReLU}(\nabla V(x)^T \hat{f}(x) + \alpha V(x))}{\| \nabla V(x) \|_2 ^2}
% \end{aligned}
% \end{equation}
% where $\hat{f}: \R^n\rightarrow\R^n$ is the nominal dynamics and $V: \R^n\rightarrow\R$ is a scalar positive definite Lyapunov function. This equation projects $\hat{f}(x)$ onto the equilibrium point. By choosing different design structures for the Lyapunov function $V$, the authors listed a series of stable neural dynamics models. 
% The model with following choice of $V(x)$ is proved to be globally exponentially stable to the equilibrium $x = 0$: 
% \begin{equation}
% \label{eq:PDICNN}
% V(x) = \sigma_k(g(x) - g(0)) + \epsilon \|x\|_2^2.
% \end{equation}
% where $\sigma_k$ is a positive convex non-decreasing function with $\sigma_k(0) = 0$, $g$ is input-convex neural network (ICNN), and $\epsilon$ is a constant. 

% This structure strongly enforces the Lyapunov function to be convex and positive definite, and hence an exponentially stable and trainable model can be obtained from such a "positive definite ICNN". Similarly one can have ICNN or multi-layer perceptron (MLP) alone as the Lyapunov function for the stable dyanmics model. 
% \subsubsection{Learning neural Hamiltonian dynamics}
% The breakthrough research in \cite{greydanus2019hamiltonian} is on learning a deep neural network, Hamiltonian Neural Networks (HNN), to model the Hamiltonian. HNN takes a pair of $\mathbf{p}$ and $\mathbf{q}$ as inputs and gives a scalar value $\mathcal{H}_{\theta}$ as the Hamiltonian, where $\theta$ represents the learnable parameters. These parameters are optimized to capture the conserved quantity from a system.  
% \begin{equation}
% \mathcal{L}_{\text{HNN}} = \left\| \frac{\partial \mathcal{H}_0}{\partial \mathbf{p}} - \frac{\mathrm{d}\mathbf{q}}{\mathrm{d}t} \right\|_2 + \left\| \frac{\partial \mathcal{H}_0}{\partial \mathbf{q}} + \frac{\mathrm{d}\mathbf{p}}{\mathrm{d}t} \right\|_2
% \end{equation}
% This work was further extended to Dissipative Hamiltonian Neural Networks DHNN in \cite{sosanya2022dissipative} to cope with more complex dynamics and extracting not only the conservation but also the dissipation, by adding a Raleigh dissipative function. 
% And it could be further generalized to the standard input-state-output form port Hamiltonian system for greater model flexibility. Nevertheless, this generalization can also result in higher risk of instability and over-fitting and hence is often implemented with some regularization methods, such as in \cite{course2020weak}. 



